SoK: Advances and Open Problems in Web Tracking

Web tracking is a pervasive and opaque practice that enables personalized advertising, retargeting, and conversion tracking. Over time, it has evolved into a sophisticated and invasive ecosystem, employing increasingly complex techniques to monitor and profile users across the web. The research community has a long track record of analyzing new web tracking techniques, designing and evaluating the effectiveness of countermeasures, and assessing compliance with privacy regulations. Despite a substantial body of work on web tracking, the literature remains fragmented across distinctly scoped studies, making it difficult to identify overarching trends, connect new but related techniques, and identify research gaps in the field. Today, web tracking is undergoing a transformation, driven by fundamental shifts in the advertising industry, the adoption of anti-tracking countermeasures by browsers, and the growing enforcement of emerging privacy regulations. This Systematization of Knowledge (SoK) aims to consolidate and synthesize this wide-ranging research, offering a comprehensive overview of the technical mechanisms, countermeasures, and regulations that shape the modern and rapidly evolving web tracking landscape. This SoK also highlights open challenges and outlines directions for future research.

==> imports.tex <==

\usepackage[all]{nowidow}
\usepackage{siunitx}
\usepackage{multirow}
\usepackage{amsmath}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage{array}
\usepackage{makecell} % optional (not required below)
\newcolumntype{Y}{>{\raggedright\arraybackslash}X}
\usepackage[most]{tcolorbox}
\usepackage{subcaption}
% \usepackage[hidelinks]{hyperref}
\RequirePackage{doi}
\usepackage{comment}
\usepackage{amssymb}
\usepackage{fancyhdr}
\usepackage{pifont} %dingautolist 
\usepackage{float}
% break urls
% \usepackage{breakurl}
\def\UrlBreaks{\do\/\do-\do_}

\renewcommand{\sectionautorefname}{Section}
\renewcommand{\subsectionautorefname}{Section}
\renewcommand{\subsubsectionautorefname}{Section}
\renewcommand{\appendixautorefname}{Appendix}
% For appendix references
\newcommand{\refappendix}[1]{\hyperref[#1]{Appendix~\ref*{#1}}}
\newcommand{\refethics}[1]{\hyperref[#1]{Ethical Considerations}}
\newcommand{\refopenscience}[1]{\hyperref[#1]{Open Science}}

% \renewcommand{\algorithmautorefname}{Algorithm}

% Prior work comparison table
\usepackage{graphicx}
\newcommand*\rot{\rotatebox{90}}
%Circles
\usepackage{tikz}
\newcommand{\emptypie}{%
\begin{tikzpicture}
 \draw (0,0) circle (.75ex);
\end{tikzpicture}%
}
\newcommand{\pie}[1]{%
\begin{tikzpicture}
 \draw (0,0) circle (.75ex);\fill[rotate=90] (.75ex,0) arc (0:#1:.75ex) -- (0,0) -- cycle;
\end{tikzpicture}%
}
\newcommand{\xmark}{\ding{55}}%

% \usepackage{xspace}
% % Add a period to the end of an abbreviation unless there's one
% % already, then \xspace.
% \makeatletter
% \DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
% \def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

% \def\eg{e.g\onedot}\def\Eg{E.g\onedot}
% \def\ie{i.e\onedot} \def\Ie{I.e\onedot}
% \def\cf{c.f\onedot} \def\Cf{C.f\onedot}
% \def\etc{etc\onedot} \def\vs{vs\onedot}
% \def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
% \def\etal{et al\onedot}
% \makeatother

\newcommand{\todo}[1]{\textcolor{red}{[#1]}}
\newcommand{\subscript}[2]{$#1 _ #2$}

\setlength{\doublerulesep}{2.5pt}

\newif{\ifanonymous}
\anonymoustrue{} % hide or show authors and other parts of the paper that should not appear at submission time


%% Gaps and Open Problem Boxed Frame
\newcommand{\gap}{\textbf{Gap}:}
\newcommand{\openproblem}{\textbf{Open Problem}:}

\usepackage[strict]{changepage}
\usepackage{framed}
\usepackage{color}

\definecolor{cosmiclatte}{rgb}{1.0, 0.97, 0.91}
\definecolor{darkred}{HTML}{AE4132}
\definecolor{lightred}{HTML}{FAD9D5}

% keywords search criteria
\newenvironment{exclusionkeywordbox}{%
  \def\FrameCommand{%
    {\color[HTML]{f8cecc}\vrule width 2pt}%
    \colorbox[HTML]{f8cecc}%
  }%
  \MakeFramed{\advance\hsize-\width\FrameRestore}%
  \noindent\hspace{-4.55pt}%
  \begin{adjustwidth}{}{7pt}%
}
{%
\end{adjustwidth}\endMakeFramed%
}

\newenvironment{keywordbox}{%
  \def\FrameCommand{%
    {\color[HTML]{d5e8d4}\vrule width 2pt}%
    \colorbox[HTML]{d5e8d4}%
  }%
  \MakeFramed{\advance\hsize-\width\FrameRestore}%
  \noindent\hspace{-4.55pt}%
  \begin{adjustwidth}{}{7pt}%
}
{%
\end{adjustwidth}\endMakeFramed%
}

% open problems
\newenvironment{opbox}{%
  \vspace{-8pt}%
  \def\FrameCommand{%
    {\color{darkred}\vrule width 2pt}%
    \colorbox{lightred}%
  }%
  \MakeFramed{\advance\hsize-\width\FrameRestore}%
  \noindent\hspace{-4.55pt}%
  \begin{adjustwidth}{}{2pt}%
  \openproblem%
}
{%
\end{adjustwidth}\endMakeFramed%
\vspace{-8pt}%
}


% gaps
\newenvironment{gapbox}{%
  \def\FrameCommand{%
    {\color{darkgray}\vrule width 2pt}%
    \colorbox{lightgray}%
  }%
  \MakeFramed{\advance\hsize-\width\FrameRestore}%
  \noindent\hspace{-4.55pt}%
  \begin{adjustwidth}{}{7pt}%
  \gap%
}
{%
\end{adjustwidth}\endMakeFramed%
}



% Defense deployment

\newcommand{\dNative}{\ding{108}} % in-browser
\newcommand{\dExt}{\ding{117}} % extension
\newcommand{\dTool}{\ding{109}} % offline/list tool
\newcommand{\dServer}{\ding{115}} % server/network/protocol/OS
\newcommand{\dNo}{\textemdash} % no/unknown industrial defense


% Tracker capabilities

% Circle fills (light pastels)
\definecolor{capIncBg}{HTML}{DBEAFE}
\definecolor{capExeBg}{HTML}{FEE2E2}
\definecolor{capObsBg}{HTML}{FEF3C7}
\definecolor{capStoBg}{HTML}{CCFBF1}
\definecolor{capShaBg}{HTML}{EDE9FE}

% Circle borders
\definecolor{capIncBd}{HTML}{93C5FD}
\definecolor{capExeBd}{HTML}{FCA5A5}
\definecolor{capObsBd}{HTML}{FCD34D}
\definecolor{capStoBd}{HTML}{5EEAD4}
\definecolor{capShaBd}{HTML}{C4B5FD}

\newcommand{\capsym}[3]{%
  \tikz[baseline=-0.55ex]{%
    \node[circle, fill=#1, draw=#2, line width=0.4pt,
          inner sep=0pt, minimum size=2.1ex,
          font=\fontsize{8}{8}\selectfont\bfseries\sffamily,
          text=black]{#3};}}

\newcommand{\symInclusion}{\capsym{capIncBg}{capIncBd}{I}}
\newcommand{\symExecution}{\capsym{capExeBg}{capExeBd}{E}}
\newcommand{\symObservation}{\capsym{capObsBg}{capObsBd}{O}}
\newcommand{\symStorage}{\capsym{capStoBg}{capStoBd}{T}}
\newcommand{\symSharing}{\capsym{capShaBg}{capShaBd}{S}}





% Icons for tracking mechanisms

\newlength{\iconsize}
\setlength{\iconsize}{0.9em}
 
\newcommand{\iconURL}{\raisebox{-0.15em}{\includegraphics[height=\iconsize]{figures/icons/url.png}}}
\newcommand{\iconFingerprint}{\raisebox{-0.15em}{\includegraphics[height=\iconsize]{figures/icons/fingerprint.png}}}
\newcommand{\iconCookie}{\raisebox{-0.15em}{\includegraphics[height=\iconsize]{figures/icons/cookie.png}}}
\newcommand{\iconJS}{\raisebox{-0.15em}{\includegraphics[height=\iconsize]{figures/icons/js.png}}}
\newcommand{\iconPrivacy}{\raisebox{-0.15em}{\includegraphics[height=\iconsize]{figures/icons/privacy.jpg}}}
\newcommand{\iconBehavioral}{\raisebox{-0.15em}{\includegraphics[height=\iconsize]{figures/icons/behavioral.png}}}
\newcommand{\iconSC}{\raisebox{-0.15em}{\includegraphics[height=\iconsize]{figures/icons/sc.png}}}

\newcommand{\iconAdBlock}{\raisebox{-0.15em}{\includegraphics[height=\iconsize]{figures/icons/block.png}}}
\newcommand{\iconCNAME}{\raisebox{-0.15em}{\includegraphics[height=\iconsize]{figures/icons/cname.png}}}



\newcommand{\iconBlocklist}{\raisebox{-0.15em}{\includegraphics[height=\iconsize]{figures/icons/blocklist.png}}}
\newcommand{\iconExtension}{\raisebox{-0.15em}{\includegraphics[height=\iconsize]{figures/icons/extension.png}}}
\newcommand{\iconTool}{\raisebox{-0.15em}{\includegraphics[height=\iconsize]{figures/icons/tool.png}}}



% Browser icons
\newcommand{\iconIE}{\raisebox{-0.3em}{\includegraphics[height=1.6em]{figures/icons/ie.png}}}
\newcommand{\iconEdge}{\raisebox{-0.3em}{\includegraphics[height=1.6em]{figures/icons/edge.png}}}
\newcommand{\iconFirefox}{\raisebox{-0.3em}{\includegraphics[height=1.6em]{figures/icons/firefox.png}}}
\newcommand{\iconSafari}{\raisebox{-0.3em}{\includegraphics[height=1.6em]{figures/icons/safari.png}}}
\newcommand{\iconChrome}{\raisebox{-0.3em}{\includegraphics[height=1.6em]{figures/icons/chrome.png}}}
\newcommand{\iconBrave}{\raisebox{-0.3em}{\includegraphics[height=1.6em]{figures/icons/brave.png}}}





% Defense Goals

% Detection and Blocking
\definecolor{cellred}{RGB}{252,235,235}
% Signal Reduction and Obfuscation
\definecolor{cellyellow}{RGB}{255,253,230}
% Regulation compliance
% Incentives
\definecolor{cellpink}{RGB}{243,230,248}
% Expectations
\definecolor{cellblue}{RGB}{230,241,253}
% Responsibilities
\definecolor{cellgreen}{RGB}{232,250,235}



\definecolor{cellempty}{RGB}{242,242,248}
\newcommand{\ec}{\cellcolor{cellempty}}
\newcommand{\rh}{\rule[-0.9em]{0pt}{2.0em}}
\newcommand{\cellsym}[1]{\parbox[c][2.0em][c]{\linewidth}{\centering #1}}




% \usepackage[landscape,margin=0.35in]{geometry}
\usepackage{calc}
\usepackage[table]{xcolor}



% TBD to create a warning at compilation (i.e., to not forget to edit later)
\newcommand{\TBD}[2]{\errmessage{#1}{[#2]}}
% \newcommand{\TBD}[1]{\errmessage{TBD}{\color{red}{[#1]}}}

%% Students
\newcommand{\yash}[1]{\textcolor{red}{[\textbf{Yash Vekaria}: #1]}}
\newcommand{\yohan}[1]{\textcolor{olive}{[\textbf{Yohan Beugin}: #1]}}
\newcommand{\shaoor}[1]{\textcolor{blue}{[\textbf{Shaoor Munir}: #1]}}

%% Professors
\newcommand{\alexandros}[1]{\textcolor{cyan}{[\textbf{AK}: #1]}}
\newcommand{\franzi}[1]{\textcolor{magenta}{[\textbf{Franziska Roesner}: #1]}}
\newcommand{\gunes}[1]{\textcolor{yellow}{[\textbf{Güneş Acar}: #1]}}
\newcommand{\jason}[1]{\textcolor{brown}{[\textbf{Jason Polakis}: #1]}}
\newcommand{\nataliia}[1]{\textcolor{cyan}{[\textbf{Nataliia Bielova}: #1]}}
\newcommand{\nick}[1]{\textcolor{green}{[\textbf{Nick Nikiforakis}: #1]}}
\newcommand{\pierre}[1]{\textcolor{orange}{[\textbf{Pierre Laperdrix}: #1]}}
\newcommand{\sebastian}[1]{\textcolor{pink}{[\textbf{Sebastian Zimmeck}: #1]}}
\newcommand{\steven}[1]{\textcolor{purple}{[\textbf{Steven Englehardt}: #1]}}
\newcommand{\umar}[1]{\textcolor{teal}{[\textbf{Umar Iqbal}: #1]}}
\newcommand{\zubair}[1]{\textcolor{violet}{[\textbf{Zubair Shafiq}: #1]}}


\newcommand{\para}[1]{\smallskip \noindent \textbf{#1}}
\newcommand{\parait}[1]{\smallskip \noindent \textit{#1}}

%Logos affiliations
\newcommand{\ucDavis}{\raisebox{2pt}{\includegraphics[width=30pt]{figures/logos/uc-davis.pdf}}}
\newcommand{\uwMadison}{\includegraphics[height=10pt]{figures/logos/uw-madison.pdf}}
\newcommand{\radboud}{\includegraphics[height=10pt]{figures/logos/radboud.pdf}}
\newcommand{\inria}{\includegraphics[height=10pt]{figures/logos/inria.pdf}}
\newcommand{\cnrs}{\includegraphics[height=10pt]{figures/logos/cnrs.pdf}}
\newcommand{\washU}{\includegraphics[height=10pt]{figures/logos/washU.jpg}}
\newcommand{\ncstate}{\raisebox{2pt}{\includegraphics[width=30pt]{figures/logos/ncstate.pdf}}}
\newcommand{\stonybrook}{\includegraphics[height=10pt]{figures/logos/stonybrook.pdf}}
\newcommand{\uic}{\includegraphics[height=10pt]{figures/logos/uic.pdf}}
\newcommand{\uwashington}{\includegraphics[height=8pt]{figures/logos/uwashington.pdf}}
\newcommand{\wu}{\includegraphics[height=10pt]{figures/logos/wu.pdf}}
\newcommand{\independent}{\raisebox{2pt}{$\dagger$}}
